ORES: Lowering Barriers with Participatory Machine Learning in Wikipedia

Algorithmic systems---from rule-based bots to machine learning classifiers---have a long history of supporting the essential work of content moderation and other curation work in peer production projects. From counter-vandalism to task routing, basic machine prediction has allowed open knowledge projects like Wikipedia to scale to the largest encyclopedia in the world, while maintaining quality and consistency. However, conversations about how quality control should work and what role algorithms should play have generally been led by the expert engineers who have the skills and resources to develop and modify these complex algorithmic systems. In this paper, we describe ORES: an algorithmic scoring service that supports real-time scoring of wiki edits using multiple independent classifiers trained on different datasets. ORES decouples several activities that have typically all been performed by engineers: choosing or curating training data, building models to serve predictions, auditing predictions, and developing interfaces or automated agents that act on those predictions. This meta-algorithmic system was designed to open up socio-technical conversations about algorithms in Wikipedia to a broader set of participants. In this paper, we discuss the theoretical mechanisms of social change ORES enables and detail case studies in participatory machine learning around ORES from the 5 years since its deployment.

==> Makefile <==
figures = \
		figures/edit_review_filters_screenshot.tex \
		figures/ores_architecture.tex \
		figures/ores_activity.tex \
		figures/ores_data_user.tex \
		figures/prediction_error_for_anons_and_newcomers.tex \
		figures/wikilabels_screenshot.tex \
		figures/ORES_precache_request_rate_201804.png \
		figures/ORES_report_mistakes_table.png \
		figures/ORES_request_activity_201804_week_vs_4hours.png \
		figures/anon_damaging_gb_vs_svc.pdf \
		figures/natural_damaging_gb_vs_svc.pdf \
		figures/newcomer_damaging_gb_vs_svc.pdf \
		figures/ORES_architecture.pdf \
		figures/ores_data_user_diagram.pdf

parts = \
		parts/abstract.tex \
		parts/authors.tex \
		parts/body.tex \
		parts/copyright.tex \
		parts/util.tex \
		parts/metadata.tex

sections = \
		sections/1_introduction.tex \
		sections/2_related_work.tex \
		sections/3_design_rationale.tex \
		sections/4_the_ores_system.tex \
		sections/5_innovations_in_openness.tex \
		sections/6_adoption_patterns.tex \
		sections/7_case_studies.tex \
		sections/8_conclusions_and_future_work.tex \
		sections/9_acknowledgements.tex \
		sections/appendix.tex


halfaker2018ores.pdf: halfaker2018ores.tex \
		$(figures) $(parts) $(sections) refs.bib acmart.cls
	rubber --pdf halfaker2018ores.tex

anon2018ores.pdf: anon2018ores.tex \
		$(figures) $(parts) $(sections) refs.bib acmart.cls
	rubber --pdf anon2018ores.tex

halfaker2018ores.with_font.pdf: halfaker2018ores.pdf
	ps2pdf13 -dPDFSETTINGS=/prepress halfaker2018ores.pdf halfaker2018ores.with_fonts.pdf

figures/anon_damaging_gb_vs_svc.pdf: figures/anon_damaging_gb_vs_svc.svg
	rsvg-convert -f pdf -o figures/anon_damaging_gb_vs_svc.pdf figures/anon_damaging_gb_vs_svc.svg

figures/natural_damaging_gb_vs_svc.pdf: figures/natural_damaging_gb_vs_svc.svg
	rsvg-convert -f pdf -o figures/natural_damaging_gb_vs_svc.pdf figures/natural_damaging_gb_vs_svc.svg

figures/newcomer_damaging_gb_vs_svc.pdf: figures/newcomer_damaging_gb_vs_svc.svg
	rsvg-convert -f pdf -o figures/newcomer_damaging_gb_vs_svc.pdf figures/newcomer_damaging_gb_vs_svc.svg

figures/ORES_architecture.pdf: figures/ORES_architecture.svg
	rsvg-convert -f pdf -o figures/ORES_architecture.pdf figures/ORES_architecture.svg

figures/ores_data_user_diagram.pdf: figures/ores_data_user_diagram.svg
	rsvg-convert -f pdf -o figures/ores_data_user_diagram.pdf figures/ores_data_user_diagram.svg


==> figures/edit_review_filters_screenshot.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=.45\textwidth]{figures/Screenshot_of_Edit_review_filters}
  \caption{A screenshot of the Edit Review Filters interface with ORES score-based filters}
  \label{fig:edit_review_filters_screenshot}
\end{figure}


==> figures/ores_architecture.tex <==
\begin{figure*}[h]
  \centering
  \includegraphics[width=.95\textwidth]{figures/ORES_architecture}
  \caption{ORES architectural overview}
  \label{fig:ores_architecture}
\end{figure*}


==> figures/ores_report_mistakes.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=.45\textwidth]{figures/ORES_report_mistakes_table}
  \caption{A slice of the ORES report mistakes table in Wikidata.}
  \label{fig:ores_report_mistakes}
\end{figure}


==> parts/authors-redacted.tex <==
\author{Redacted F. Review}
\orcid{1234-5678-9012-3456}
\affiliation{%
  \institution{XXXXXXX}
  \streetaddress{XXXXXXX}
  \city{XXXXX}
  \state{XX}
  \postcode{12345}
  \country{XXX}}
\email{XXXX@XX.XX}

\author{Redacted G. Review}
\orcid{1234-5678-9012-3456}
\affiliation{%
  \institution{XXXXXXX}
  \streetaddress{XXXXXXX}
  \city{XXXXX}
  \state{XX}
  \postcode{12345}
  \country{XXX}}
\email{XXXX@XX.XX}

\renewcommand{\shortauthors}{XXX et al.}

==> sections/old/6_adoption_patterns.tex <==
When we designed and developed ORES, we were targeting a specific problem: expanding the set of values applied to the design of quality control tools to include a recent understanding of the importance of newcomer socialization.  We do not have any direct control of how developers chose to use ORES.  This is one of the key characterics of employing a ``hearing to speech'' strategy.  We hypothesize that, by making edit quality predictions available to all developers, we would lower the barrier to experimentation in this space.   After we deployed ORES, we implemented some basic tools to showcase the, but we observed a steady adoption of our various prediction models by external developers in current tools and through the development of new tools.

When we first released ORES, there was a wave of adoption in tools that were already used by Wikipedians.  Machine predictions proved useful as an addition to already-engineered systems used to support content patrolling work.  While this dynamic itself is fascinating, for the purposes of this paper, we focus on the development of new tools that use ORES that may not have been developed at all otherwise.  For example, the Wikimedia Foundation's product department developed a complete redesign on MediaWiki's Special:RecentChanges interface that implements a set of powerful filters and highlighting.  They took the ORES Review Tool (one of our demo interfaces) to it's logical conclusion with an initiative that they referred to as Edit Review Improvements.\footnote{\url{http://enwp.org/:mw:Edit_Review_Improvements}}  In this interface, ORES scores are prominently featured at the top of the list of available filters, and they have been highlighted as one of the main benefits of the new interface to the editing community.

When we first developed ORES, English Wikipedia was the only wiki that we are aware of that had a fully-automated bot that used machine prediction to automatically revert obvious vandalism \cite{carter2008cluebot}.  After we deployed ORES, several wikis developed such bots of their own using ORES.  For example, SeroBOT in Spanish Wikipedia\footnote{\url{https://es.wikipedia.org/wiki/Usuario:SeroBOT}} and Dexbot in Persian Wikipedia\footnote{\url{https://fa.wikipedia.org/wiki/User:Dexbot}} now automatically revert edits that ORES predicts are damaging with high confidence. 

One of the most noteworthy new applications of ORES is the suite of tools developed by Sage Ross to support the Wiki Education Foundation's\footnote{\url{https://wikiedu.org/}} activities.  Their organization supports classroom activities that involve editing Wikipedia.  They develop tools and dashboards that help students contribute successfully and to help teachers monitor their students' work.  Ross has recently published about how he interprets meaning from ORES' article quality models \cite{ross2016visualizing} (an example of re-appropriation) and he has used the article quality model in their new editor support dashboard\footnote{\url{https://dashboard-testing.wikiedu.org}} in a novel way.  Specifically, Ross's tool\footnote{\url{https://dashboard-testing.wikiedu.org}} uses our feature injection system (see Section~\ref{sec:innovations_in_openness}) to suggest work to new editors.  This system asks ORES to score a student's draft article and then asks ORES to reconsider the predicted quality level of the article with \emph{one more header}, \emph{one more image}, \emph{one more citation}, etc. -- tracking changes in the prediction and suggesting the largest positive change to the student.  In doing so, Ross built an intelligent user interface that can expose the internal structure of a model in order to recommend the most productive development to the article---the change that will most likely bring it to a higher quality level. This type of adoption pattern is interesting in what it achieves but also how it balances concerns around quality control efficiency and newcomer socialization in a totally novel way.  By helping student editors learn how to structure their articles to match Wikipedians expectations, Ross's tool has the potential to both improve newcomer socialization and minimize the burden for patrollers.


==> sections/old/7_case_studies.tex <==
When we first deployed ORES, we reached out to several different wiki communities and invited them to test the system for use in patrolling for vandalism.  Before long, our users began filing false-positive reports on wiki pages of their own design --- some after our request, but mostly on their own.  In this section, we describe three cases where our non-technical end-users independently developed these false-positive reporting pages and we describe how they used them to understand ORES, the roles of automated quality control in their own spaces, and to communicate with us about model bias.

\subsection{Patrolling/ORES (Italian Wikipedia)}
Italian Wikipedia was one of the first wikis where we deployed basic edit quality models.  Our local collaborator, who helped us develop the language specific features, User:Rotpunkt, created a page for ORES\footnote{\url{https://it.wikipedia.org/wiki/Progetto:Patrolling/ORES}} with a section for reporting false-positives (``falsi positivi'').  Within several hours, Rotpunkt and a few other editors noticed some trends.  These editors began to collect false positives under different headers representing themes they were seeing.  Through this process, editors from Italian Wikipedia were effectively performing an inductive, grounded theory-esque exploration of ORES errors.

One of the themes they identified fell under the header: ``corrections to the verb for \emph{have}'' (``correzioni verbo avere'').  It turns out that the word ``ha'' in Italian translates to the English verb ``to have''.  In English and many other languages, ``ha'' signifies laughing, and it generally is not a phrase found in encyclopedic prose. In addition, most language versions of Wikipedia tend to have at least some amount of English-language vandalism.  We had built a common feature in the damage model called ``informal words'' that captured these types of patterns.  But in this case, it was clear that in Italian ``ha'' should not carry signal of vandalism, while ``hahaha'' still should. Because of the work of Rotpunkt and his collaborators in Italian Wikipedia, we were able to recognize the source of this issue (a set of features intended to detect the use of \emph{informal language} in articles) and to remove ``ha'' from that list for Italian Wikipedia.

\subsection{PatruBOT (Spanish Wikipedia)}
Soon after we released support for Spanish Wikipedia, a volunteer developer made a bot to automatically revert edits using ORES's predictions for the ``damaging'' model (PatruBOT).  This bot was not running for long before our discussion spaces were bombarded with confused Spanish-speaking editors asking us why ORES did not like their work.  We struggled to understand the complaints until someone told us about PatruBOT. 

After inspection, we found that this case highlighted the tradeoffs between precision/recall and false positives/negatives---a common issue with machine learning applications. We concluded that PatruBOT's threshold for reverting was too sensitive. ORES reports a classification and a probability score, but it is up to the developers to decide if, for example, the bot will only auto-revert edits classified as damage with a .90, .95, .99, or higher likelihood estimate. A higher threshold will minimize the chance a good edit will be mistakenly auto-reverted, but also increase the chance that a bad edit will not be auto-reverted.  Ultimately, our view was that each volunteer community should decide where to draw the line between false positives and false negatives, but we could help inform their discussion.

The Spanish Wikipedians who were concerned with these issues began a discussion about PatruBOT's activities and blocked the bot until the issue was sorted. Using wiki pages, they organized an crowdsourced evaluation of the fitness of PatruBOT's behavior\footnote{\url{https://es.wikipedia.org/wiki/Wikipedia:Mantenimiento/Revisi\%C3\%B3n_de_errores_de_PatruBOT\%2FAn\%C3\%A1lisis}}.  This evaluation and discussion is ongoing, \footnote{\url{https://es.wikipedia.org/wiki/Wikipedia:Caf\%C3\%A9\%2FArchivo\%2FMiscel\%C3\%A1nea\%2FActual\#Parada_de_PatruBOT}} but it shows how stakeholders do not need to have an advanced understanding in machine learning evaluation to meaningfully participate in a sophisticated discussion about how, when, why, and under what conditions such classifiers should be used. Because of the API-based design of the ORES system, no actions are needed on our end once they make a decision, as the fully-automated bot is developed and governed by Spanish Wikipedians.

\subsection{Bias against anonymous editors}
\input{figures/prediction_error_for_anons_and_newcomers}
Shortly after we deployed ORES, we received reports that ORES's damage detection models were overly biased against anonymous editors.  At the time, we were using Linear SVM\footnote{\url{http://scikit-learn.org/stable/modules/generated/sklearn.svm.LinearSVC.html}} estimators to build classifiers, and we were considering making the transition towards ensemble strategies like GradientBoosting and RandomForest estimators.\footnote{\url{http://scikit-learn.org/stable/modules/ensemble.html}}  We took the opportunity to look for bias in the error of estimation between anonymous editors and newly registered editors.  By using our feature injection/interrogation strategy (described in Section~\ref{sec:innovations_in_openness}), we could ask our current prediction models how they would change their predictions if the exact same edit were made by a different editor.

Figure~\ref{fig:prediction_error_for_anons_and_newcomers} shows the probability density of the likelihood of ``damaging'' given three different passes over the exact same test set, using two of our modeling strategies.  Figure~\ref{fig:natural_damaging_gb_bs_svc} shows that, when we leave the features to their natural values, it appears that both models are able to differentiate effectively between damaging edits (high-damaging probability) and non-damaging edits (low-damaging probability) with the odd exception of a large amount of non-damaging edits with a relatively high-damaging probability around 0.8 in the case of the Linear SVM model.  Figures~\ref{fig:anon_damaging_gb_bs_svc} and \ref{fig:newcomer_damaging_gb_bs_svc} show a stark difference.  For the scores that go into these plots, characteristics of anonymous editors and newly registered editors were injected for all of the test edits.  We can see that the GradientBoosting model can still differentiate damage from non-damage while the Linear SVM model flags nearly all edits as damage in both cases.

Through the reporting of this issue and our subsequent analysis, we were able to identify the weakness of our estimator and show that an improvement to our modeling strategy mitigates the problem.  Without such a tight feedback loop, we most likely would not have noticed how poorly ORES's damage detection models were performing in practice.  Worse, it might have caused vandal fighters to be increasingly (and inappropriately) skeptical of contributions by anonymous editors and newly registered editors---two groups of contributors that are already met with unnecessary hostility\footnote{\url{http://enwp.org/:en:Wikipedia:IPs_are_human_too}}\cite{halfaker2013rise}.


==> sections/summary_of_changes.tex <==
\pagebreak
\section{Summary of Changes}

Thank you to the reviewers for your critiques and suggestions.  

When considering our revision of this paper, we focused carefully on the AC's advice: ``I believe the reviewers are just looking for the paper to support the claims more carefully and more fully."  It's clear to us that this paper did not make it clear that we intend to position the paper as a systems paper and that our use of ``case studies" was to give early impressions of usage.  It also seems clear to us that the AC and some reviewers wanted to see more of the socio-technical side of ORES represented in the paper.  

For resubmission, we've produced a substantial rewrite of the paper.  In this version of the paper, you'll find a more clear discussion of the broader system under review.  We explicitly call out the socio-technical components of ORES (our engineering team and the processes we've engaged in when consulting with Wikipedia editors).  

The new version of the paper also makes it clear that we built ORES and our engineering team is responsible for managing the socio-technical support of processes around ORES.

This version of the paper also leaves out all mention of causal claims around ``increasing reflection" and instead focuses on actually telling stories about what that reflection looks like and what it means for the development of open, collaborative machine learning systems.  To avoid confusion around the term ``case studies", we have renamed these sections ``demonstrative cases" and we have included substantial discussion of what exactly these cases are intended to demonstrate.  

We've also brought a much more nuanced discussion of decoupling that the ORES system supports.  We specifically contrast the tightly coupled pattern of our collaborative model design and development pattern with the highly decoupled pattern of appropriation of models using the service.

We brought in some detail from the appendix that reviewers asked for.  E.g., discussion of the Wiki Labels system and discussion of how feature injection and threshold optimization work.  But we didn't merely bring these technical details in, we also included demonstrative cases that explain their origin and show how they are used in practice. 

With these changes, the paper has gained substantial length pre-references.  The majority of this additional length is due to the increased focus on the socio-technical dynamics surrounding ORES, the demonstrative cases, and an extended discussion section.  We thank you for your time and consideration.
